The Option Value of Contract Duration: Evidence from the U.S. Timber Market

This study quantifies how contract duration influences buyers' willingness-to-pay (WTP) when they hold real options that allow them to flexibly time consumption in response to changing market conditions. Using contract data from the US timber industry, we show that buyers delay consumption to manage payoff risk. This behavior generates heterogeneous WTP across buyers. We use structural estimation to uncover the key parameters underlying the incentive to delay consumption. Using these estimates, we conduct counterfactual simulations to measure how longer contract durations shift WTP and to clarify the boundary conditions linked to project size, buyer composition, and market trends. The counterfactual simulations reveal that extending contract duration from 3 to 4 years raises seller revenue by 9-13%, with effects amplified for larger projects and high-type buyers during the upward market trend.

==> figuretable/entry_stage_estimate.tex <==

\begin{tabular}[t]{lcc}
\toprule
Oral & $\lambda_{l}$ & $\lambda_{s}$\\
 & 0.161 & 0.153\\
 & {}[0.067] & {}[0.067]\\
 &  & \\
Sealed bid & $\lambda_{l}$ & $\lambda_{s}$\\
 & 0.142 & 0.142\\
 & {}[0.016] & {}[0.016]\\
\bottomrule
\end{tabular}


==> figuretable/number_of_active_bidders.tex <==

\begin{tabular}[t]{lllllll}
\toprule
Num of active bidders & 1 & 2 & 3 & 4 & 5 & 6\\
Oral & 98 & 109 & 65 & 23 & 7 & 4\\
Sealed & 51 & 28 & 18 & 10 & 4 & 1\\
\bottomrule
\end{tabular}


==> slides_figure/slides_counterfactual_large_symmetric.tex <==
\begin{tabular}[t]{cccrrrr}
\toprule
 Participants & 12 quarters & 16 quarters\\
\midrule
 (S, S) &  386.438 & 455.004\\
 (L, L) &  145.133 & 149.361\\
 (S, S, S) &  407.560 & 477.361\\
 (L, L, L) & 119.421 & 115.310\\
\bottomrule
\end{tabular}


==> slides_figure/slides_counterfactual_small_symmetric.tex <==
\begin{tabular}[t]{crrrr}
\toprule
 Participants  & 12 quarters & 16 quarters\\
\midrule
 (S, S) &  264.210 & 290.437\\
  (L, L) & 82.204 & 84.092\\
 (S, S, S) & 281.541 & 308.452\\
 (L, L, L) & 64.708 & 67.151\\
\bottomrule
\end{tabular}

==> text_sections/01-1_introduction.tex <==
\section{Introduction}\label{sec:introduction}

Advance selling is a strategy used in many industries, such as concerts, sports events, vacation packages, and natural resource markets, where buyers pay for goods or services before they are consumed. This approach allows sellers to manage demand uncertainty and improve their revenue by selling early. While much of the research on advance selling focuses on topics about pricing and buyer behavior, one important aspect has received little attention: the length of time buyers are given to use their purchase. Does giving buyers more time to use what they bought make them willing to pay more? And how does this affect the seller’s earnings? Using data from U.S. timber auctions, this paper explores how the length of the consumption period impacts buyers’ valuations and bidding strategies, shedding light on how sellers can design contracts and selling mechanisms to increase revenue.

In the context of advance selling, products can generally be divided into two categories: those tied to specific scheduled events, like concerts or sports games, and those that allow flexible consumption within a designated period, such as an annual pass for an amusement park, car leases, and natural resource leases. This paper focuses on the latter category, where the length of the consumption period plays a critical role in shaping buyers’ valuations and sellers’ revenue. Our timber auction data provide a unique setting to study the role of consumption periods in advance selling. In these auctions, buyers acquire the right to harvest timber, but they are not required to immediately cut and transport it. Instead, they are granted a fixed consumption period—typically three years—to decide the timing of their actions. During this period, buyers face uncertainty about future lumber prices, which significantly impacts their valuations and harvest decisions. This structure mirrors advance selling contexts where buyers secure future consumption rights but must navigate uncertainty about the eventual payoff. As highlighted in the literature, longer consumption periods allow buyers to reduce uncertainty by waiting for favorable market conditions, such as higher lumber prices, thereby increasing their willingness-to-pay at the purchase stage. Indeed, public forest managers receive public comments requiring longer lease duration in timber sales, which indicates the importance of our investigation from the practical perspective as well.\footnote{See SECTION 5463.1 in  \href{https://www.federalregister.gov/documents/2020/12/18/2020-27580/forest-management-decision-protest-process-and-timber-sale-administration}{the document}  of the Forest Management Decision Protest Process and Timber Sale Administration. [accessed July 7, 2024]}

Another key feature of this study is its focus on auctions as a mechanism for advance selling, a topic that remains underexplored in the existing literature. In traditional advance selling contexts, sellers often combine advance price with spot price to exploit buyers’ valuation uncertainty and maximize revenue. However, when sellers lack knowledge about buyers’ payoffs, setting optimal prices becomes challenging—especially when buyers are heterogeneous in their future payoffs. Auctions play a crucial role in such cases because of their price discovery effect. This paper offers practical guidance for sellers on choosing the more effective auction format—oral or sealed-bid—to maximize revenue under various conditions regarding lumber price, length of consumption period, and the size of products. By exploring the interaction between buyer heterogeneity, auction design, and the advance selling framework, this study provides actionable insights into how sellers can strategically structure auctions to enhance revenue outcomes.

We begin our analysis by studying data from the Bureau of Land Management (BLM), U.S. Department of Interior and Federal Reserve Economic Data (FRED). Our data indicate that timber harvesting decisions are influenced by lumber prices and the remaining lease duration. A significant amount of timber is harvested when lumber prices rise, whereas harvesting is postponed when lumber prices are low or the lease expiration date is not imminent. These dynamic incentives in the harvesting phase connect to outcomes in the auctions. The auction data suggests that longer lease duration raises bidders' valuation, as the winning bidder can delay harvesting in anticipation of higher lumber prices. We also found that different types of buyers exhibit distinct patterns in both cutting and bidding behaviors, indicating that changes in consumption periods and auction designs have heterogeneous impacts on the shapes of buyers' value. 


Motivated by these salient features of the data, we propose a structural model that combines bidding in auctions with post-auction actions. First, our model considers oral auctions. Bidders are divided into two types: loggers and manufacturer sawmills. Each type has different participation probabilities and faces different distributions of value. Second, the cutting stage follows the first stage oral auctions, and we interpret the second stage as a real option model, where the flexibility to choose when to harvest timber adds value to the auction prize. For this stage, we construct the dynamic single-agent model in which the winning bidder chooses when and how much to cut timber upon realized timber prices. A single agent prefers higher timber prices, but she must remove all timber by the deadline. These incentives characterize the observed cutting patterns. Note that bidders' valuation in the first stage stems from the continuation value in the post-auction cutting stage.



We bring the model to the data on timber auctions and timber cutting. First, we use the variations in timber prices and the amounts of cut timber to estimate parameters underlying the dynamic cutting behavior in the spirit of \cite{rust1987optimal}. Second, we estimate the composition of loggers to sawmill manufacturers leveraging the observed number of auction participants, proposing a simple estimation method similar to \cite{kong2020not}, which does not rely on the specific entry model. Third, using the estimated dynamic model and entry parameters, we recover the distribution of bidders' value based on the bidding equilibrium. 

Our estimation results reveal key differences between loggers and sawmills, highlighting the importance of bidder heterogeneity in timber auctions. At the cutting stage, sawmills benefit from lower costs and less sensitivity to lumber prices, reflecting their operational efficiencies. In the bidding stage, sawmills show higher and more dispersed valuations, making them high-type buyers. Additionally, both bidder types are more likely to participate in oral auctions, likely due to larger tracts being assigned to this format. Together, these findings underline the role of bidder heterogeneity and auction design in shaping outcomes, providing a foundation for the counterfactual analysis of auction formats and consumption periods.

We then use the estimated model primitives to perform welfare analysis. Our counterfactual analysis demonstrates that extending the consumption periods significantly increases sellers’ revenue by enhancing bidders’ valuations, particularly through the flexibility to adjust harvesting decisions based on future market conditions. This effect is more pronounced for stronger bidders, such as sawmills, whose valuations respond more robustly to longer horizons. However, the magnitude of revenue gains varies across auction formats, competition intensity, and bidder heterogeneity. For instance, sealed-bid auctions tend to amplify revenue growth when the second-highest bidder belongs to the low-type, while oral auctions excel in more competitive settings such that high-type buyers lose. Additionally, larger tracts magnify the revenue benefits of longer consumption periods due to the higher strategic value of deferring harvests. These findings highlight the critical role of contract length and auction design in shaping revenue outcomes, providing insights for sellers managing advance selling strategies under various market conditions.


The insights from this paper extend to industries offering flexible consumption periods, such as ticket sales and leasing. A longer consumption period provides a real option—the flexibility to use the product when desired, essentially allowing for delayed consumption. This option holds significant value when future needs are uncertain. For instance, consider an amusement park selling annual passes: customers purchase the right to visit the park anytime within a year. Those uncertain about their future availability might prefer the option of a longer validity period, even if it comes at a higher price. This flexibility, analogous to the option to delay timber harvests in our study, influences the perceived value of the pass. Therefore, sellers and lessors must understand how the real option element within these contracts shapes consumer valuations and purchase decisions. Our methods offer valuable insights into how sellers can structure the length of ticket validity periods or lease terms to maximize revenue, even with limited knowledge of individual customer preferences or future circumstances. Understanding the effect of the length of consumption period enables sellers to better cater to diverse customer needs and ultimately enhance their revenue potential.

Our study also connects to another category of advance selling products—those tied to specific scheduled events. Although these products have a pre-specified consumption timing, the time length between purchase and event date introduces a layer of uncertainty that can affect buyer valuations. For example, suppose that the purchase date is closer to the event date. In that case, buyers are less likely to encounter unexpected circumstances (such as accidents or scheduling conflicts) that might prevent them from attending the event, thereby increasing the perceived value of the ticket. This implies a negative correlation between the length of the purchase period and the product’s value, contrasting with the positive correlation observed for flexible consumption periods.

The rest of the paper is organized as follows. The remainder of this section discusses the related literature. Section \ref{sec:data} describes the data and its background. Section \ref{sec:model} develops the model which explains the empirical findings. Section \ref{sec:estimation} describes estimation details and discusses estimation results. Section \ref{sec:counterfactual} describes the counterfactual algorithm, performs counterfactual simulations, and discusses counterfactual results. Section \ref{sec:conclusion} concludes.

==> text_sections/01-2_literature.tex <==
\paragraph{Related literature}
This paper relates to several strands of literature: advance selling, auctions followed by state-dependent payoffs, and empirical applications of real options theory. First, advance selling has emerged as a vital area of marketing research. \cite{shugan2000advance} show that offering advance sales alongside spot sales can yield revenues comparable to first-degree price discrimination, as it enables sellers to capitalize on buyers' uncertainty about future valuations. \cite{xie2001electronic} extend this framework by incorporating capacity constraints, staggered arrivals of buyers, refund policies, buyer risk aversion, and various other factors. For a comprehensive overview, one can refer to \cite{xie2009advance}, and the literature continues to grow (e.g., \cite{yu2015rationing}; \cite{cachon2017advance}; \cite{seo2020pricing}). An extension of advance selling is inter-temporal or dynamic pricing, which allows sellers to adjust prices across multiple purchase periods in response to evolving buyer valuations as the event date approaches, as explored by \cite{lazarev2013welfare}, \cite{soysal2012demand}, and \cite{williams2022welfare}.

Despite these advances, existing research has largely overlooked the role of the consumption period’s length, even though its importance is acknowledged in \cite{shugan2000advance} and \cite{xie2001electronic}.\footnote{The contract term and its formation are also discussed in empirical bargaining literature \citep{lee2021structural}.} Our paper addresses this gap by examining how the duration of the consumption period influences valuation uncertainty and buyers’ consumption decisions, and consequently, affects sellers’ revenue. Furthermore, previous studies often assume that sellers have accurate knowledge of the distribution of future buyer valuations, which may not hold in practice. As \cite{sainam2010consumer} suggest, introducing auctions can help reveal buyers’ willingness-to-pay and guide optimal advance selling strategies. By considering advance selling auctions, our analysis demonstrates how to estimate buyer valuations when faced with payoff uncertainty, thereby contributing new insights into pricing and timing strategies in advance selling contexts.

Second, recent empirical auction research increasingly examines how the design of auctions followed by state-dependent payoffs influences bidders’ initial strategies. Examples include \cite{ordin2019investment}; \cite{bhattacharya2022bidding}; \cite{kong2022multidimensional}, and they draw data on oil and gas lease auctions. Those auctions involve ex-post payoff uncertainty: future oil and gas prices determine the value of extracted resources and shape drilling incentives. Since bidders pay a predetermined share of production as royalties, sellers face a moral hazard problem—if prices rise, buyers have a greater incentive to drill and produce, but if prices fall, buyers may under-produce despite holding valuable extraction rights and sellers may receive less royalties.

Timber auctions also feature state-dependent payoffs, as future lumber prices determine the ultimate profitability of the purchased asset. Unlike oil and gas leases, however, many Bureau of Land Management (BLM) timber auctions require a lump-sum payment upfront, with no subsequent payments contingent on realized production. While this removes the moral hazard issue associated with output-based transfers, it does not render the environment trivial. The value of the asset still depends on evolving market conditions, and the temporal constraints on resource extraction impose their own strategic considerations, affecting both bidders’ ex-ante valuations and ex-post actions.

Timber auctions have long been central to empirical auction research, offering insights into risk aversion, auction design, bidder asymmetries, and more (\cite{athey2001information}; \cite{haile2001auctions}; \cite{li2003timber}; \cite{lu2008estimating}; \cite{athey2011comparing}; \cite{roberts2013should}; \cite{li2015affiliation})\footnote{For a comprehensive survey, see \cite{hortaccsu2021empirical}.}. Our study extends this literature by showing how changes to the contract’s consumption period alter bidder asymmetries and interact with auction formats. In doing so, we complement the literature on auction with state-dependent payoff by demonstrating that, even in the absence of moral hazard, the interplay between market-driven valuations and contractual timing can substantially influence post-auction strategies and equilibrium bidding behavior.


Third, our empirical findings contribute to the literature that applies real options theory to actual data. Examples include \cite{collard2013demand}, \cite{kellogg2014effect}, \cite{agerton2020learning}, and \cite{herrnstadt2024drilling}. Especially, \cite{herrnstadt2024drilling} is close to our article, as both papers study the effects of deadline lengths on agents' decisions on when to consume time-limited objects. The key difference between our paper and \cite{herrnstadt2024drilling} is that our paper quantifies the effects of deadlines on competition by leveraging bidding data, which is not addressed in \cite{herrnstadt2024drilling}. Real options theory is also applied to timber harvest data in the field of agricultural economics. Examples include \cite{rucker1988harvest}, \cite{insley2005solving}, and \cite{alvarez2007optimal}. One can refer to \cite{hildebrandt2011investment} and \cite{yousefpour2012review} for comprehensive surveys of this literature. Our article contributes to the literature by applying a dynamic structural model to harvest records. To the best of our knowledge, this paper is the first to quantify the effects of contract terms on both timber harvesting and bidding behaviors. 

\begin{comment}
There are several papers investigating auctions with contingent payment. (See \cite{skrzypacz2013auctions} for the review of theoretical papers.) \cite{lewis2011procurement} investigate the welfare effect of multiple-attributes bid auction in which bidders submit project cost and the length of time for procurement construction. Conditioning on that the firms do not face uncertainty about completion time, they show that scoring auction will improve construction speed and commuters' welfare more than the loss from the increased construction cost. Using oil and gas lease auction data in New Mexico, \cite{bhattacharya2022bidding} study how auction mechanism affects the bidding behavior through its effect on incentive of drilling when the winner faces uncertainty about its revenue. They show that lower royalty rate plays a role as insurance and gives an incentive of drilling the tracts while reducing seller's revenue from the production itself. With the same data, \cite{ordin2019investment} simulates the effects of different revenue tax schemes on post-auction drilling activity and the seller's revenue. While bidders cannot choose royalty rate in \cite{bhattacharya2022bidding} and \cite{ordin2019investment}, \cite{kong2022multidimensional} study the case in which both bonus payment and royalty are choice variables. Using oil lease auction data in Louisiana, they show that the bidders with inefficient productivity become more aggressive as they can choose higher royalty, which exacerbates adverse selection and moral hazard, and leads to lower revenue for the seller than fixed-royalty auctions. 
\end{comment}




==> text_sections/02_data.tex <==
\section{Data}\label{sec:data}
We analyze auctions organized by the Bureau of Land Management (BLM), U.S. Department of Interior, which is responsible for managing federal forests. In this section, we describe the timber sales process, our data, and key empirical findings.

\subsection{Timber sales process}
BLM manages forests in several states including  Oregon, Montana, Indiana, Colorado, Wyoming, California, and Utah. As timber growth in the forests reaches a certain point, BLM holds auctions to determine which company will cut the grown timber. BLM adopts different selling mechanisms for different timber forests: bilateral negotiations, oral auctions, and first-price sealed-bid auctions. Our analysis focuses on auctions since the scale of bilateral negotiations is limited. We display the monetary scale of each selling format in Section \ref{subsec:data_description}. For payment rules, BLM adopts different systems for each sale: scale sales and lump-sum sales. Bidders submit unit prices in scale sales, and the total payment equals the product of submitted unit prices and actual harvested quantities. In lump-sum sales, bidders submit total prices for the tract, and the payment equals the submitted prices regardless of the volume of harvested timber. 

Before the auctions, BLM presents the prospectus for the auctioned forests. From the prospectus, the interested bidders observe the estimated volume of timber for each species, reserve prices, bidding rule, terms of lease including lease duration and down-payment, and the characteristics of the forests, such as locations and road conditions. Interested bidders have the opportunity to cruise the forests and prepare bids. 

Participants in the auctions are typically local loggers and sawmill manufacturers. Loggers and sawmill manufacturers have different positions in the wood supply chain. Loggers mainly cut timber and transport it to processing facilities called sawmills, where sawmill manufacturers process the transported wood into lumbers and veneers. Lumbers and veneers are mainly purchased by home-building companies as input goods. In short, loggers are upstream, and sawmill manufacturers are downstream in the supply chain. 

After the auctions, BLM grants the winning bidder the right to remove timber from the tract. The contract is time-limited, implying that the winning bidder must cut all timber by the deadline. The lease duration is typically 36 months. If the winning bidder faces events such as weather, fire closure, and other related conditions that interrupt operating time, BLM may extend the lease duration. However, it is rare to see the extension so the winning bidder has to prepare for removing every timber by the due date.

\subsection{Data description}\label{subsec:data_description}
This paper relies on a data set of timber auctions organized between 2012Q2 and 2023Q1 by the Bureau of Land Management (BLM), U.S. Department of Interior. BLM data consists of two parts of records: transaction data and contract data. The former includes auction results such as the number of bidders, winning prices, reserve prices, and, if any, the second-highest bids. One can observe other auction characteristics, including the number of acres of timber tract and lease duration. From the latter data, one can observe the records of timber harvests, such as the timing and the volume of timber removal. We also draw data on lumber market prices from Federal Reserve Economic Data (FRED). As we see in the later section, lumber market prices relate to timber removals.

Table \ref{tb:summary_statistics_of_entry_and_bidding_stage} reports the summary statistics of BLM data. The market mechanisms chosen by the BLM for its sales of standing timber are auctions for about 47\% of its sales and negotiated contracts for the remaining 53\%. The BLM employs two auction mechanisms: ascending (oral) auctions and first-price sealed-bid auctions. Of the auctioned sales, oral auctions constitute the majority at 73\% (306 out of 418), while sealed-bid auctions account for the remaining 27\% (112 out of 418). The choice of auction mechanism for each lease is influenced by feedback from participants, with anecdotal evidence suggesting a general preference for oral auctions. However, oral auctions were partially suspended during the COVID-19 pandemic. Bilateral negotiation is typically used for smaller tracts, with negotiation partners selected on a rotational basis. On average, oral auctions involve larger tracts (3,977 mbf) than sealed-bid auctions (2,587 mbf), whereas negotiated contracts are associated with much smaller tracts, averaging 221 mbf.

On average, $2.16$ ($2.03$) bidders enter the oral (first-price sealed-bid) auctions, while $10.35$ ($5.25$) bidders are counted as potential participants. One cannot observe the number of potential bidders from the raw data, and it is defined as the potential bidders to be the number of unique bidders in the neighborhood of 10 km that participated in some auction (sealed bid or open outcry) organized by BLM between 2012Q2 and 2023Q1. In terms of seller's revenues, both winning and reserve prices are higher in oral auctions than in sealed-bid auctions.


This table also highlights the presence of asymmetric buyers in the auctions. The variable ``Manufacturer'' is a dummy variable indicating whether the winner is a sawmill, with sawmills accounting for 62\% of the winners. Although the exact number of sawmills and loggers near the auctioned tracts is unknown, it is likely that loggers outnumber sawmills in this industry\footnote{In Oregon, approximately 700 logging companies exist (\hyperlink{https://www.dnb.com/business-directory/company-information.logging.us.oregon.html}{Dun \& Bradstreet}, accessed December 13, 2024), compared to around 100 sawmills (\hyperlink{https://www.whereorg.com/businesses/sawmills-or}{Whereorg.com}, accessed December 13, 2024)}. Considering this, Table \ref{tb:summary_statistics_of_entry_and_bidding_stage} suggests that sawmills, on average, represent high-type buyers with stronger valuations relative to loggers.


The variable ``Lumpsum'' is a dummy variable that takes value one if the payment does not depend on actual volumes of cut timber but estimated timber volumes. Table \ref{tb:summary_statistics_of_entry_and_bidding_stage} indicates that 86\% of oral auctions adopt a lumpsum format. The difference between actual timber volumes and estimated timber volumes is summarized in Table \ref{tb:summary_statistics_of_diff_actualestimated}. On average, the discrepancies are small across both oral and sealed-bid formats, with mean differences ranging from -0.11 to -0.03 in oral auctions and -0.09 to -0.06 in sealed-bid auctions. The small standard deviations indicate that actual outcomes closely align with estimates, particularly in value terms, where differences are concentrated around zero. These results justify the common adoption of lump-sum contracts, as the predicted timber quantities provide reliable benchmarks for payment determination. Figure \ref{fg:diff_actualestimated} presents the histogram of the difference between actual cut timber values and estimated values, and the difference concentrates around zero.

Panel (b) of Table \ref{tb:summary_statistics_of_entry_and_bidding_stage} summarizes the contract data in BLM records. Cutting most frequently occurs ($14.59$ times in the lease duration) in oral auctions than in the other formats. The variable  ``Cutting delay'' represents the observed removal time after the awarded date, and it takes $21.99$ months, whereas the average contract term is $32.43$ months in oral auctions. It suggests that the timing of timber removals concentrates around the end of the lease duration. We discuss more details about the timing of timber removals in the following Section \ref{subsubsec:fact_findings}. Moreover, the “Revised contract term,” which captures lease extensions, averages 36.72 months in oral auctions and 31.16 months in sealed-bid auctions, suggesting an average extension of approximately 4 months. However, it remains unclear whether this extension significantly benefits buyers in terms of their operational or financial outcomes.

Figure $\ref{fg:lumber_price_trend}$ describes the time-trend of lumber market prices. The number in this figure represents the index value for lumber market prices. One can observe that lumber prices fluctuate across periods, especially during the COVID-19 pandemic (after 2020). During this period, housing prices soar because people must stay home and have incentives to invest in their houses.  

\begin{landscape}
\begin{table}[ht!]\small
\begin{centering}
      \caption{Summary statistics}      \label{tb:summary_statistics_of_entry_and_bidding_stage} 
      \subfloat[Entry and bidding stage]{\input{figuretable/summary_statistics_of_entry_and_bidding_stage}}\\ 
      \subfloat[Cutting stage]{\input{figuretable/summary_statistics_of_cutting_stage}}\\
\end{centering}
 \footnotesize
  \textit{Sources}: 2012Q2 and 2023Q1 by the Bureau of Land Management (BLM), U.S. Department of Interior.
\end{table} 
\end{landscape}

\begin{table}[h]\small
  \begin{center}
      \caption{Summary statistics of difference between estimate and actual cuts}
      \label{tb:summary_statistics_of_diff_actualestimated} \input{figuretable/summary_statistics_of_diff_actualestimated}
  \end{center}\footnotesize
  Note: This table displays the difference between actual and estimated cutting amounts, standardized by the predicted quantities at the auction stage. The table reports basic statistics for four measures: acres, ccf (hundred cubic feet), mbf (thousand board feet), and transaction value. 
\end{table} 


\begin{figure}[h]
\begin{center}
\includegraphics[height = 0.4\textheight]{figuretable/actual_minus_estimated_value.png}
\end{center}
\caption{The difference b/w actual and estimated cut timber values}\footnotesize
\label{fg:diff_actualestimated}
\end{figure}


\begin{figure}[h]
\begin{center}
\includegraphics[height = 0.4\textheight]{figuretable/lumber_price_trend.png}
\end{center}
\caption{Lumber price trends}\footnotesize
\textit{Sources}: Federal Reserve Economic Data (FRED).
\label{fg:lumber_price_trend}
\end{figure}


\subsection{Fact findings}\label{subsubsec:fact_findings}
We discuss the empirical patterns, which motivate our policy questions and structural model. The first finding is that the entry decisions do not relate to auction characteristics. Second, we find that the longer lease duration raises bidders' value. Third, the timing of removal completions concentrates on the lease expiration date. 

\paragraph{Exogenous entry}
We estimate Poisson regression models to assess the factors explaining the number of active bidders, focusing on 265 auctions in which more than two active bidders exist.
Table \ref{tb:poisson_result_num_of_active_bidders} shows estimation results of the number of active bidders and participation rates on observed auction-level characteristics. The covariates include the lease duration, the auction format, lumber prices, the COVID-19 period dummy, reserve prices, and the size of the timber forest. We do not find any statistically significant relationship between bidders' entry and observed characteristics. 
This implies that there is a priori no self-selection of bidders in the sense that the auction format and contract term do not affect the decision of a bidder to participate, as in \cite{lu2008estimating}.
Based on this finding, we focus on the post-entry and post-auction stages leaving the pre-auction stage as exogenous.

\begin{table}[h]
  \begin{center}
      \caption{Poisson regressions of the number of active bidders}
      \label{tb:poisson_result_num_of_active_bidders} 
      \input{figuretable/poisson_result_num_of_active_bidders}
  \end{center}\footnotesize
 Note: This table presents Poisson regression results for the number of active bidders and the percentage of active bidders as dependent variables. ``Contract term'' represents the lease duration in months, while ``Sealed'' is a dummy variable equal to 1 for sealed-bid auctions. The interaction term ``Contract term × Sealed'' captures the combined effect of lease duration and auction format. Additional covariates include ``Lumber pric'' for market timber prices, ``Covid dummy'' accounting for the COVID-19 period, ``Reserve price'' indicating the auction's minimum bid, and ``Acres'', representing tract size. Standard errors are reported in parentheses. The analysis is based on 265 observations, with RMSE values provided for model fit. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\end{table} 

\begin{landscape}
\begin{table}[h]
{\footnotesize
  \begin{center}
      \caption{Regressions of log of winning bids and reserve prices}
      \label{tb:regression_result_log_highest_bid_reserve_price} 
      \input{figuretable/regression_result_log_highest_bid_reserve_price}
  \end{center}}\footnotesize
  Note: This table presents regression results for the natural logarithm of winning bids and reserve prices as dependent variables. Explanatory variables include ``Contract term'', indicating the lease duration in months; ``Sealed'', a dummy variable equal to 1 for sealed-bid auctions; and ``Contract term × Sealed'', an interaction term capturing the joint effect of lease duration and sealed-bid format. Other covariates include ``Lumber price'', representing market timber prices; ``Covid dummy'', a variable accounting for the COVID-19 period; ``Num of active bidders'', the number of participants actively bidding; ``Acres'' and ``Mbf'', which capture tract size in acres and thousand board feet, respectively; and ``Manufacturer'', a dummy variable equal to 1 if the buyer is a sawmill manufacturer. Standard errors are reported in parentheses. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively. 
\end{table} 
\end{landscape}
%この基本統計とかプロットの意図は、伐採量の意思決定をしているのかどうかを見るというもので、偏りがないなら切る切らないの２択から選択しているというモデルの正当化になるため


\paragraph{Effects of lease duration on bidders' value}
Table \ref{tb:regression_result_log_highest_bid_reserve_price} shows regression results of the log of winning bids and reserve prices on observed auction-level characteristics. 
We find a strong positive relationship between winning bids and contract term lengths for oral auctions, whereas negative for sealed-bid auctions. 
Extending a contract term length by one month increases a winning bid by about 5\% for oral auctions, but decreases by at most 0.9\% for sealed-bid auctions. Thus, the heterogeneity across auctioned tracts is quite well captured by not only the lumber price, number of active bidders, reserve price, and volume measured by acres and mbf as in \cite{lu2008estimating}, but also the contract duration. The negative coefficient of the interaction term between the contract term and the sealed-bid format dummy suggests that the benefits of a longer contract term on seller revenue are more limited under the sealed-bid format. We explore the intuition behind this finding in the counterfactual section.




\paragraph{Timing of removal completion}
% 価格とManufacturerダミーで回帰分析。ここでAsymmetryがあるかどうかを議論する。Manufacturerの方が価格に敏感。Manufacturerの方がカットコストが高い可能性あり。

\begin{figure}[h!]
  \begin{center}
 \subfloat[$25\%$ of progress]{\includegraphics[keepaspectratio, scale=0.8]{figuretable/cutting_completition_timing_0.25.png}}
  \subfloat[$50\%$ of progress]{\includegraphics[keepaspectratio, scale=0.8]{figuretable/cutting_completition_timing_0.5.png}}\\
  \subfloat[$75\%$ of progress]{\includegraphics[keepaspectratio, scale=0.8]{figuretable/cutting_completition_timing_0.75.png}}
  \subfloat[$100\%$ of progress]{\includegraphics[keepaspectratio, scale=0.8]{figuretable/cutting_completition_timing_1.png}}
  \caption{Distribution of cutting progress}
  \label{fg:time_hist_100} 
  \end{center}
  \footnotesize
   Note: These figures illustrate histograms of the timing of timber removal completion as a proportion of the contract period, where 0 indicates the start of the contract (awarded date) and 1 represents the end of the contract (expiration date). Panels (a)–(d) show the distribution of completion timing for 25\%, 50\%, 75\%, and 100\% progress in timber removal, respectively. 
\end{figure} 

\begin{table}[h!]
  \begin{center}
      \caption{Regressions of quarter-level cutting amounts}
      \label{tb:regression_result_transaction_cut_amount} 
      \input{figuretable/regression_result_transaction_cut_amount}
  \end{center}\footnotesize
  Note: This table presents regression results for quarter-level cutting amounts. The dependent variables are measured in three units: ``Transaction mbf'' represents the volume of timber harvested in thousand board feet (mbf), ``Transaction Acres'' refers to the acreage of timber harvested, and ``Transaction Value'' denotes the monetary value of harvested timber. Explanatory variables include ``Lumber Price'', indicating the market price of timber during the quarter, ``Manufacturer'', a dummy variable equal to 1 if the buyer is a sawmill manufacturer, and controls for the total tract size measured in mbf, acres, and value. Standard errors are reported in parentheses. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively. 
\end{table} 


Figure \ref{fg:time_hist_100} illustrates the histogram of time spent at each level of cutting progress. For example, Panel (a) shows that one tends to harvest only 25\% of designated timber even when half of the contract duration has elapsed. The mode of the histogram shifts progressively from left to right as cutting progress increases, as shown in Panels (b) and (c). Panel (d), which focuses on completed timber removals, indicates that most harvesting is completed near the contract expiration date. This pattern underscores how bidders often delay timber cutting until later in the contract period, likely to account for market price uncertainty and operational constraints. 

To investigate what affects the timing of harvest, we run regressions of quarter-level cutting amounts on quarter-level lumber prices and their interaction with heterogeneous agents' types. The dependent variables include three measures of harvest amounts; mbf, acres, and monetary value. The mbf is a forestry term for ``1000 board feet''. From Table \ref{tb:regression_result_transaction_cut_amount},
we find a strong positive relationship between lumber prices and cutting behavior for three cutting amount measures. 
When lumber prices are high, buyers are likely to cut and sell more timbers. This suggests that dynamic allocation decisions are conditional on time-varying information such as timber prices in a finite horizon determined by the contract term. The results also reveal distinct differences in cutting behavior between buyer types. Sawmill manufacturers harvest larger volumes of timber at given quarter compared to loggers conditional on lumber price and tract size.



==> text_sections/03_model.tex <==
\section{Model}\label{sec:model}
In this section, we propose a structural model and discuss its equilibrium outcome. Our model has two sequential stages: the bidding stage and the cutting stage. In the bidding stage, both loggers and sawmill manufacturers submit their bids. Then, the winning buyer in the bidding stage obtains the right to consume timber, and she faces a single-agent dynamic problem: when and how much timber to cut until the lease expires. In the following Section \ref{subsec:setup}, we provide more details of our model settings and introduce notations. In Section $\ref{subsec:analysis}$, we derive solutions to our model, which we bring to data in the following estimation part. 

\subsection{Setup}\label{subsec:setup}

\paragraph{Bidding stage}
We model bidding in oral auctions with $n_k$ bidders for each auction $k$, whereas we do not model entry and assume that the number of bidders $n_k$ is exogenous. Auction $k$ has characteristics $\boldsymbol{x}_k$, which includes the contract period $T_k$, the size of timber forest $u_{k0}$,  and current lumber prices $p_0$. Bidders belong to one of two types: logger $l$ or sawmill manufacturer $s$. Each bidder $i$ has private information regarding the private value of the timber forest denoted by $v_{ik}:=\xi_{ik}V^{m(i)}_0(\boldsymbol{x}_k)$, which consists of idiosyncratic factor $\xi_{ik}$ and common factor $V^{m(i)}_0(\boldsymbol{x}_k)$ for type $m(i)\in \{l,s \}$ of bidder $i$. The idiosyncratic factor $\xi_{ki}$ reflects private information of bidder $i$ in auction $k$ that differentiates her from another. For example, it could include factors such as the bidder’s specific expertise, management efficiency, opportunity cost, or access to other complementary resources that are not explicitly modeled but influence their willingness-to-pay. The common factor $V^{m(i)}_0(\boldsymbol{x}_k)$ is determined within the dynamic optimization problem in the cutting stage mentioned later. Different bidders have different facilities for processing timber, so they anticipate different values when facing the same timber forest. We assume that each type of bidder has different distributions of $\xi_{ik}$. The logger bidder draws $\xi_{ik}$ from the distribution $F_l(\cdot)$, whereas the sawmill manufacturer bidder draws $\xi_{ik}$ from the distribution $F_s(\cdot)$. The common factor $V^{m(i)}_0(\boldsymbol{x}_k)$ captures the values that do not vary across bidders but vary across types denoted by $m(i) \in \{l,s \}$. The amounts of timber to be cut and lumber market prices are common among bidders, which leads to common value for bidders within the same type. Based on their private value, each bidder $i$ submits bid $b_{ik}$ for auction $k$. As we consider oral auctions, the winner is defined by the bidder who submits the highest bid among the participants and the winners' payment is equal to the highest bid. 


\paragraph{Cutting stage}
After winning auction $k$, the winner of the auction solves a dynamic single-agent problem with finite periods $T_k$.
At the begin of each period $t \in \{1,2,...,T_k\}$, winner $i$ observes state variable $s_{kt}$. 
The state variable in period $t$ includes lumber prices $p_t$ and the size of uncut areas $u_{kt}$, i.e., $s_{kt}=(p_t,u_{kt})$. By definition, initial state $s_{k0}$ in period 0 is equivalent to auction characteristics $\boldsymbol{x}_{k}$.
Depending on the state at each period, winner $i$ decides how much timber to harvest. The amount of cut timbers at period $t$ is denoted by $q_{kt}u_{kt}$. We define $q_{kt}\in \{0, 0.25, 0.5, 0.75, 1\}$ as the ratio of cut timber to all standing timber at the initial period. We discretize the ratio to model action as a discrete choice for computational tractability. For example, $q_{kt}=0.5$ implies that the winning bidder cuts 50 \% of timber in the tract. Based on the actions taken by the winner and the value of the current state variable, the transition of the state variable in the next period is determined as follows:
\begin{align}
    u_{k,t+1} &= u_{kt} - u_{k0}q_{kt};  \\
    p_{t+1} &\sim f(\cdot|p_{t}) ,
\end{align}
where $f(\cdot|p_{t})$ captures the distribution of future lumber price conditional on the current price $p_t$. We assume that $u_{k1}=u_{k0}$, where $u_{k0}$ is the size of timber forest defined as a part of auction characteristics $\boldsymbol{x}_k$. It is not hard to justify this assumption since our data suggests in Section \ref{sec:data} that the estimated timber volume does not much differ from the actual timber volume. We also assume that timber prices are not influenced by the timber supply in our data, as the auctions in BLM data represent only a relatively small portion of the overall timber supply.

In each period, winner $i$ in auction $k$ obtains the following temporal deterministic payoff by cutting $q_{kt}$ percent of the timber tract.
\begin{align}
    q_{kt}u_{kt}(\gamma_{m(i)}p_t - c_{1m(i)} - c_{2m(i)}q_{kt}u_{kt})+\varepsilon^{q_{kt}}_{ikt},
\end{align}
where $\gamma_{m(i)}$ represents type-specific sensitivity to lumber market prices, $c_{1m(i)}$ is type-specific marginal cutting cost for winner $i$'s type $m(i)$, and $c_{2m(i)}$ is type-specific nonlinear cutting cost. The last term $\varepsilon^{q_{kt}}_{ikt}$ denotes action-specific demand shock and $\varepsilon_{ikt}=\varepsilon^{q_{kt}}_{ikt}$. Since the winner must remove all timber from the tract, $\sum_{t=1}^{T_{k}}q_{kt}=1$ must hold.


\subsection{Analysis}\label{subsec:analysis}
In this section, we solve the model backwardly. First, we define the maximization problem faced by the winner and derive the continuation value at the initial time period. Second, using the computed continuation value, we solve the bidding problem in the auction stage. 

% \begin{itemize}
%     \item The following is a memo of Otani tasks on dynamic parts.
%     \item Action is binary, i.e., cutting some amount or not.
%     \item State discretization is based on the level of cutting amount, not to ratio because cutting sunk cost must be heterogeneous. For example, while the cutting ratio is the same, the costs of cutting 1ha and cutting 100ha must be different. Or cutting sunk cost should have some parametric form of cutting amounts.
%     \begin{itemize}
%         \item The remaining amount of timbers
%         \item Timber prices
%     \end{itemize}
%     \item \textcolor{blue}{[TBA] Terminal stage at $T$ value function}
%     \item \textcolor{blue}{[TBA] Stage at $T-1$ value function}
%     \item Choice specific value function
%     \item Conditional choice probability
%     \item We solve the model backwardly by applying the finite period version of \cite{rust1987optimal}.
%     \item Learning on $p_{t}$.
% \end{itemize}

\paragraph{Cutting stage}
In the cutting stage, winner $i$ in auction $k$ aims to maximize her expected future payoff. In other words, she solves the following Bellman equation:

\begin{align}\label{eq:bellman_equation}
    V^{m(i)}_t(s_{kt}, \varepsilon_{ikt}) =& \max_{q_{kt}}q_{kt}u_{kt}(\gamma_{m(i)}p_t - c_{1m(i)} - c_{2m(i)}q_{kt}u_{kt}) + \varepsilon^{q_{kt}}_{ikt} \\
    &+  \beta E_{\varepsilon_{ikt+1}}\left[V^{m(i)}_{t+1}(s_{k,t+1}, \varepsilon_{ikt+1}|s_{kt}, \varepsilon_{ikt},q_{kt})\right], \nonumber\\
    & \text{subject to }\begin{cases}
    q_{kt} \leq 1 - \sum^{t-1}_{\tau=1}q_{k\tau},& \text{ if }t<T_k \\
    q_{kt} = 1 - \sum^{t-1}_{\tau=1}q_{k\tau},& \text{ if }t=T_k 
    \end{cases},\nonumber
\end{align} 
where $\beta$ is a discount factor.
Since buyers have to remove all remaining timbers at the terminal period due to the rule, $V^{m(i)}_T(s_{kT}, \varepsilon_{ikT}) = u_{kT}(\gamma_{m(i)}p_T - c_{1m(i)} - c_{2m(i)}u_{kT})$. The first two terms in Equation \eqref{eq:bellman_equation} represent the temporal payoff from cutting $q_{kt}$, whereas the third term captures the expected continuation value. The expectation is taken with respect to lumber prices in the next period. The constraints suggest that one must harvest all timber within the lease duration. To construct the tractable model, we follow \cite{rust1987optimal} and assume the conditional independence assumption that $\operatorname{Pr}\left(s_{kt+1}, \varepsilon_{ikt+1} \mid s_{kt}, \varepsilon_{ikt}, q_{kt}\right)=\operatorname{Pr}\left(s_{kt+1} \mid s_{kt}, q_{kt}\right) \cdot \operatorname{Pr}\left(\varepsilon_{ikt+1} \mid s_{kt}\right)$ and that action-specific demand shock $\varepsilon^{q_{kt}}_{ikt}$ follows the type-I extreme value distribution $f(\varepsilon^{q_{kt}}_{ikt})$. 
Then, using the part of Equation \eqref{eq:bellman_equation}, we define the integrated value function as
\begin{align}
    V^{m(i)}_t(s_{kt}) =& \int_{\varepsilon_{ikt}}\biggl[\max_{q_{kt}}q_{kt}u_{kt}(\gamma_{m(i)}p_t - c_{1m(i)} - c_{2m(i)}q_{kt}u_{kt}) + \varepsilon^{q_{kt}}_{ikt} \nonumber\\
    &+  \beta E_{\varepsilon_{ikt+1}}\left[V^{m(i)}_{t+1}(s_{k,t+1}|s_{kt},q_{kt})\right]\biggr] f(\varepsilon_{ikt}) d\varepsilon_{ikt}, \nonumber\\
    =&\int_{\varepsilon_{ikt}^{q}}[v_{ikt}^{q_{kt}}(s_{kt}) + \varepsilon^{q_{kt}}_{ikt}] f(\varepsilon_{ikt}) d\varepsilon_{ikt},\nonumber
\end{align}
where $v_{ikt}^{q_{kt}}(s_{kt})$ is the choice-specific continuation value.
Finally, we obtain the conditional choice probability that the winner chooses $q_{kt}$ as follows:
\begin{align}
    \operatorname{Pr}(q_{kt}|s_{kt}) &=  \frac{\exp\left(v_{ikt}^{q_{kt}}(s_{kt})\right)}{\sum_{q'_{kt}}\exp\left(v_{ikt}^{q'_{kt}}(s_{kt}))\right)}.
\end{align}
The continuation value at the initial period $V^{m(i)}_0(s_{k0})$ determines the common part of bidders' value discussed in the previous section. 

\paragraph{Bidding stage}
Given the continuation value at the initial period $V^{m(i)}_0(\boldsymbol{x}_k)$, the bidding strategy at equilibrium is straightforward, as we consider oral auctions. All bidders have a dominant strategy of bidding up to their valuation: $b^*_{ik}=\xi_{ik}V^{m(i)}_0(\boldsymbol{x}_k)$. Therefore, the payment by the winner at equilibrium is equivalent to the second-highest value among the participants. 

==> text_sections/04_estimation.tex <==
\section{Estimation}\label{sec:estimation}
The goal of this section is to identify and estimate the structural parameters. We have two-type of parameters to be identified and estimated: the parameters underlying the dynamic part and the parameters in the auction part. The dynamic parameters include the sensitivity to lumber market prices and marginal cutting costs. The auction parameters include the distribution of private value for loggers and sawmill manufacturers. We also need to recover parameters regarding the fraction of each type among the auction participants. This information is crucial for simulating first-price sealed-bid auctions in the counterfactual analysis.

Our BLM data shows the number of bidders, the winner's identity and type, and the winning price for each oral auction. Based on this information, we construct the number of potential loggers and sawmill manufacturers who may enter the auctions. For timber removals, we observe the amount of cut timber every quarter for each timber tract. From FRED data, we observe lumber market prices quarterly. The variations in lumber prices allow us to identify the price sensitivity of loggers and sawmill manufacturers, and the volume of cut timber indicates the marginal cutting costs. After identifying these dynamic parameters, we can compute the continuation value of the timber tracts. Combining this with submitted bid prices, we can identify the distribution of bidders' value. The proportion of bidder's type is identified by the variations in the number of potential and actual bidders. Leveraging our knowledge about the number of actual entrants, we do not need to use the variations in submitted bids as \cite{kong2022identification} has done.

\subsection{Estimation strategies}
\subsubsection{Dynamic parameters}
\paragraph{Cutting stage}
Recall that we model the cutting action as a discrete choice problem, where the decision is to choose from a set of possible timber reduction levels: (0, 0.25, 0.5, 0.75, 1). These values represent the proportion of the current timber amount that is removed, where 0 indicates no removal, and 1 indicates full removal, and intermediate levels indicate incremental reduction by 25\%. This specification is supported by the data construction, as the analyst observes the amount of timber cut at each quarter, reflecting aggregated cutting amounts, rather than a continuous spectrum of removal. Using the dynamic discrete choice model, we estimate the sensitivity to lumber prices $\gamma_{m}$ and the marginal cutting cost $\boldsymbol{c}_m$ for each type $m$. Our estimation relies on the Nested Fixed Point Algorithm developed by \cite{rust1987optimal}. In the inner loop of this algorithm, given an initial guess for the parameters $(\gamma_{m},\boldsymbol{c}_m)$, we compute the continuation value and choice probability starting from the terminal decision period and iteratively work backward to the initial period. In the outer loop, we update the parameters $(\gamma_{m},\boldsymbol{c}_m)$ to maximize the likelihood of the observed data. This iterative process ensures that the parameter estimates align with the observed cutting decisions and underlying dynamics.

\subsubsection{Auction parameters}
\paragraph{Entry stage}
We first estimate the fraction of type $m$ among the participants. In our application, we have two types; loggers ($l$) and sawmills ($s$). We denote type $m$ bidders' entry probability by $\lambda_m$ and $\boldsymbol{\lambda}=(\lambda_l,\lambda_s)$. This parameter directly relates to the fraction of each type, as we can express the fraction of loggers by $\frac{\lambda_l}{\lambda_l + \lambda_s}$. Outside the model, we estimate $\lambda_m$ by leveraging the information of the number of participants $n_k$ for each auction $k$. Suppose we also know the number of potential bidders for each type denoted by $N^m_k$\footnote{The information of the potential bidders is available from many sources: data from the negotiation data or Oregon DOF}. Then, the likelihood that we observe the $n_k$ participants can be expressed as follows:
\begin{align}
    \operatorname{Pr}(n_k|\boldsymbol{\lambda},n_k>0) = \sum_{j \in \{0,...,n_k\}}\frac{\operatorname{Pr}(j \text{ loggers enter}|N^l_k,\lambda_l)\operatorname{Pr}(n_k - j \text{ sawmills enter}|N^s_k,\lambda_s)}{1-\operatorname{Pr}(\text{No logger enters})\operatorname{Pr}(\text{No sawmill enters})}.\label{eq:likelihood_entry}
    \end{align}
The left-hand side in Equation \eqref{eq:likelihood_entry} represents the probability that auction $k$ has $n_k$ entrants conditional on that at least one bidder enters and the auction is not canceled. The numerator on the right-hand side indicates the probability that $j$ loggers and $n_k - j$ sawmills attend, whereas the denominator captures the probability that the auction is not canceled due to no entrants. We consider the condition that auctions are not canceled, as we cannot observe auctions with zero participants. We calculate each probability using poison distribution with parameter $\lambda_m$ and estimate the parameter by maximizing the likelihood.


\paragraph{Bidding stage}
It is also straightforward to estimate the parameters regarding the valuation from the bidding data and the estimates of dynamic parameters. Consider the event that bidder $i$ with type $m\in \{l,s\}$ wins the auction among $N$ bidders with the transaction price $\tau$. Following \cite{kong2022identification}, we can express the probability density of the event as follows:
{\footnotesize
\begin{align}
    &p(i \text{ wins with }\tau | N,V^{m}_{0}; \hat{p}_m) = \left(1-F^m(\tau|V^{m}_{0}) \right) \left[\sum_{n=0}^{N-1} \left\{ \underbrace{{n \choose N-1} \hat{p}^n_m (1-\hat{p}_m )^{N-1-n}}_{\text{probability that n loggers participate}} \right.\right.  \nonumber \\
    &\left.\left. \sum_{j \in \{1,...,N-1\}} \left(\underbrace{1\left[j \leq n \right]f^l_j(\tau|V^{l}_{0})[F^l(\tau|V^{l}_{0})]^{n-1} [F^s(\tau|V^{s}_{0})]^{N-1-n}}_{\text{logger j submits the second-highest bid}} + \underbrace{1\left[j > n \right]f^s_j(\tau|V^{s}_{0})[F^l(\tau|V^{l}_{0})]^{n} [F^s(\tau|V^{s}_{0})]^{N-2-n}}_{\text{sawmill j submits the second-highest bid}}\right)\right\}\right],
\end{align}
}where $\hat{p}_m$ is the estimate of the fraction of type $m$ bidders from the entry stage and $V^{m}_{0}$ is the continuation value computed from estimated dynamic parameters. For type $m\in \{l,s\}$, we parameterize $F^{m}(\tau|V^{m}_{0})$ as the gamma distribution with scale and shape parameters $(\mu_{m}V^{m}_{0},\sigma_{m})$ and estimate $(\mu_{m},\sigma_{m})$.


\subsection{Estimation results}

\begin{table}[!htbp]
  \begin{center}
      \caption{Estimation results}
      \label{tb:estimation_results} 
      \subfloat[Cutting stage]{\input{figuretable/cutting_stage_estimate}}
      \subfloat[Bidding stage]{\input{figuretable/bidding_stage_estimate}}
      \subfloat[Entry stage]{\input{figuretable/entry_stage_estimate}}
  \end{center}\footnotesize
  \textit{Note}: For computing standard errors, we choose 1000 bootstrap samples, each of which contains resamples of auction data.
\end{table} 

\subsubsection{Cutting stage}


Panel (a) in Table \ref{tb:estimation_results} presents the estimation results of dynamic parameters at the cutting stage. The findings suggest that sawmills exhibit lower sensitivity to lumber prices compared to loggers, as evidenced by the parameter $\gamma_s=0.065$ being smaller than $\gamma_l=0.138$. This indicates that loggers are more inclined to increase timber cutting in response to rising prices, whereas sawmills adjust their cutting activity less frequently in response to such price changes. The difference is likely due to the fact that loggers, often small businesses, lack sufficient storage capacity for harvested timber, making them more responsive to high lumber prices as an incentive to cut timber.

Additionally, the estimates indicate that loggers tend to incur higher cutting costs ($c_{1l}=25.06$) compared to manufacturers $(c_{1s}=11.91)$. This disparity can likely be attributed to differences in business size and structure. Manufacturers, who integrate logging, delivery, and processing operations, can achieve efficiencies across these stages, thereby reducing overall cutting costs. In contrast, loggers—typically smaller, independent businesses—must transport cut timber to their customers' processing facilities, introducing an additional layer of logistical inefficiency. This lack of integration adds to their operational costs, exacerbating the cost disparity between loggers and larger manufacturers.

Overall, these findings underline the importance of accounting for bidder heterogeneity when modeling timber auctions. Differences in price sensitivity and operational costs play a critical role in shaping bidders’ continuation values, which directly influence bidding strategies in the auction stage. These dynamics highlight the distinct strategic considerations faced by loggers and sawmills in both cutting and auction contexts.

%Panel (a) in Figure \ref{fg:model_fit_bidder_valuation_highest_bid} illustrates the simulated and actual path conditional on the timber prices. \textcolor{blue}{[TBA]}.

\subsubsection{Bidding stage}
Panel (b) in Table \ref{tb:estimation_results} reports estimation results of distribution parameters of bidder valuations in the bidding stage. These results indicate that sawmills have a more dispersed value distribution with higher expected value relative to loggers. The estimated parameters $\mu$ and $\sigma$ are scale and shape parameters governing gamma distribution which $\xi$ follows. Recall that $\xi$ captures heterogeneous value among bidders. Sawmills have a larger shape parameter value $\sigma_s=1.56$ than loggers, indicating larger expected value of sawmills' valuation relative to loggers, which is consistent with the findings in \cite{athey2011comparing} that sawmills are likely to be stronger bidders. Furthermore, the scale parameter value of sawmills is larger than loggers' ($3.65$ vs $0.81$). As a variance of the gamma distribution is defined by $\mu^2 \times \sigma$, this result indicates that heterogeneity among sawmills is much larger than that among loggers.


\begin{figure}[!ht]
  \begin{center}
 % \subfloat[Cutting stage \textcolor{blue}{[TBA]}]{\includegraphics[keepaspectratio, scale=0.6]{figuretable/model_fit_bidder_valuation_highest_bid.png}}
  \subfloat[Bidding stage]{\includegraphics[keepaspectratio, scale=0.7]{figuretable/model_fit_bidder_valuation_highest_bid.png}}
  \subfloat[Entry stage]{\includegraphics[keepaspectratio, scale=0.7]{figuretable/model_fit_entry_rate_num_of_active_bidders.png}}
  \caption{Model validation}
  \label{fg:model_fit_bidder_valuation_highest_bid} 
  \end{center}
  \footnotesize
  Note: These figures validate the model by comparing predicted outcomes with observed data. Panel (a) presents the probability density of the highest bids in the bidding stage, where the purple line represents the actual data, and the yellow line indicates the model-predicted distribution. Panel (b) shows the distribution of the number of active bidders in the entry stage, with observed data in purple and model predictions in yellow. 
\end{figure} 

Panel (a) in Figure \ref{fg:model_fit_bidder_valuation_highest_bid} illustrates the probability density of the highest bids in the data and prediction using estimated parameters. Both histograms display a similar pattern, with winning prices clustering around $120$ and exhibiting a rightward skew.

\subsubsection{Entry stage}

Panel (b) in Table \ref{tb:estimation_results} displays the estimated entry probability for each type of bidder. We estimate the entry probability in sealed-bid auctions as well even though we only use data from oral auctions in the subsequent analysis. This is because we simulate bidding behavior in sealed-bid auctions in our counterfactual analysis and the information of entry patterns is required there. The estimated parameters $\boldsymbol{\lambda}$ indicate that both loggers and sawmills raise their entry probability in oral auctions relative to sealed-bid auctions. We can attribute this result to the empirical evidence, shown in panel (a) of Table \ref{tb:summary_statistics_of_entry_and_bidding_stage}, that the auctioneers are likely to assign larger tracts to oral auctions. 

Panel (b) in Figure \ref{fg:model_fit_bidder_valuation_highest_bid} illustrates the proportion of active bidders in the data and prediction using estimated parameters. Predicted numbers fit well for the data.



==> text_sections/05_counterfactual.tex <==
\section{Counterfactual}\label{sec:counterfactual}
Given estimated parameters, we quantify and decompose the effects of contract length on sellers' revenue and how its effects change across selling mechanisms (auction formats). First, we simulate different contract lengths and examine how they affect the cutting behavior and result in different cutting values. Second, we compute how these different contract lengths, through their effects on cutting value, affect buyers' willingness to pay and, consequently, sellers' revenue.

\subsection{Effects of contract length on cutting value}

\begin{figure}[!ht]
  \begin{center}
 \subfloat[Logger's continuation value conditional on price grid level = 1, 2]{\includegraphics[keepaspectratio, scale=0.8]{figuretable/continuation_value_plot_logger_price_grid_1.png}\includegraphics[keepaspectratio, scale=0.8]{figuretable/continuation_value_plot_logger_price_grid_2.png}}\\
  \subfloat[Sawmill's continuation value conditional on price grid level = 1, 2]{\includegraphics[keepaspectratio, scale=0.8]{figuretable/continuation_value_plot_manufacturer_price_grid_1.png}\includegraphics[keepaspectratio, scale=0.8]{figuretable/continuation_value_plot_manufacturer_price_grid_2.png}}
  \caption{Continuation value for each contract length}
  \label{fg:continuation_value_plot} 
  \end{center}
  \footnotesize
  Note: This figure shows how the estimated continuation values in the units of $\$1000$ vary by contract length, holding either a low (price grid = 1) or intermediate (price grid = 2) lumber price environment at the time of bidding. Each colored line represents a different tract size. Panel (a) focuses on loggers, while panel (b) presents the corresponding values for sawmills. The vertical dashed line indicates the baseline contract length observed in our data.
\end{figure} 


Before proceeding to the full auction simulations, we begin by examining the baseline continuation values that underpin bidders’ valuations at the time of bidding. Figure \ref{fg:continuation_value_plot}, panel (a), displays the continuation values for loggers across varying contract lengths and tract sizes, under two distinct lumber price states (price grid level 1 for lower prices and level 2 for intermediate prices at the time of bidding). Figure \ref{fg:continuation_value_plot}, panel (b), presents the corresponding continuation values for sawmills under similar conditions. In both panels, each line represents a different cumulative tract size, illustrating how resource scale interacts with contract length and price conditions.

Several key patterns emerge from these results. First, as shown in panel (a) for loggers, extending the contract length consistently enhances continuation values, particularly in low initial price scenarios (price grid = 1). When initial prices are subdued, the option to wait for more favorable market conditions is highly valuable, causing valuations to rise markedly as the contract horizon lengthens. Under intermediate initial price conditions (price grid = 2), continuation values start from a higher baseline, and while they still increase with contract length, the marginal gains are somewhat more moderate. Panel (b) for sawmills reveals a similar trend: longer contracts provide greater flexibility to exploit future price improvements, although the incremental benefits are more enhanced compared to the loggers' scenario. This difference can be attributed to our estimation results, which indicate that sawmills are less sensitive to price fluctuations and cutting volumes. Thus, the presence of more demand shocks, represented by $\boldsymbol{\varepsilon}_{ikt}$, has a greater impact on sawmills' valuations than on loggers'

Second, tract size amplifies the influence of contract length and price state. Larger tracts command higher continuation values across all horizons, as indicated by the upward shift of curves in both panels. This pattern reflects the increased absolute gain from deferring harvest until prices improve. Greater resource availability broadens strategic options, enabling both loggers and sawmills to better time extraction decisions. Although both bidder types benefit, the shape and steepness of their valuation curves differ, highlighting that their cost structures and market strategies respond differently to temporal and price-based incentives.

Finally, comparing panels (a) and (b) shows that bidder type matters. Loggers appear more sensitive to contract extensions under low-price scenarios, experiencing sharper increases in continuation values as the horizon lengthens. Sawmills also benefit from long-term flexibility, but their valuation growth is generally smoother. These differences suggest that the interplay of contract design, market expectations, and resource endowments varies systematically across bidder types.

In sum, the evidence from Figure \ref{fg:continuation_value_plot} demonstrates that contract length, market state, and tract size jointly shape the baseline valuations that bidders bring into the auction. Longer horizons substantially increase the option value of future market conditions, larger tracts magnify potential payoffs, and distinct bidder types respond in unique ways. These findings set the stage for our subsequent counterfactual simulations, where we investigate how these underlying valuation patterns influence equilibrium bidding behavior and ultimately affect auction outcomes.

\begin{comment}
    Figure \ref{fg:continuation_value_plot} shows the effect of contract length on continuation value. 
It exhibits a clear upward trajectory, with a diminishing rate of increase as contract length extends. For shorter contract lengths, the continuation value rises steeply. This pattern suggests that extending contracts provides substantial benefits for short contracts, likely due to \textcolor{blue}{XXX}. However, as the contract length increases, the rate of growth in continuation value begins to plateau. This diminishing marginal return highlights the fact that the incremental gains in value become less pronounced beyond a certain threshold. 

Furthermore, the relationship between contract length and continuation value varies systematically across cumulative tract sizes. Larger tract sizes consistently result in higher continuation values, regardless of contract length. This indicates a scaling effect, where larger tracts inherently contribute more value, likely due to \textcolor{blue}{XXX}. 

Panel (b) of Figure \ref{fg:continuation_value_plot_manufacturer_price_grid_2} highlights a pronounced upward curvature in the relationship between contract length and continuation value for smaller cumulative tract sizes, particularly at shorter contract lengths. For cumulative tract sizes such as 9, 25, and 41, the continuation value increases rapidly as contract length extends, exhibiting steep growth. This suggests that for smaller tracts, extending contract lengths significantly enhances the perceived or actual value of the contract. The pattern likely reflects the heightened sensitivity of smaller tracts to longer-term commitments, where longer contracts provide more stability or certainty, amplifying their relative value.

However, as the contract length increases, this steep growth diminishes, and the continuation value begins to plateau, especially for intermediate and larger cumulative tract sizes. For larger tract sizes such as 104, 136, and 165, the continuation value is relatively less sensitive to contract length, exhibiting a flatter curve. This pattern indicates that the marginal benefits of extending contract length are more pronounced for smaller tract sizes, while larger tracts derive substantial value regardless of contract duration. Thus, the lower left panel underscores how contract length interacts with tract size, with smaller tracts benefiting disproportionately from initial extensions in contract length.

\textcolor{blue}{Need to mention that initial price matters in the effects of longer contract length}.
\end{comment}

\subsection{Effects of contract length on seller's revenue}
Next, we quantify how the aforementioned effects of longer consumption duration on buyers' value affect sellers' revenue. To compute the expected revenue for sellers in auctions, we derive bidding functions by following \cite{hubbard2013using}. Interested readers can refer to Appendix \ref{sec:appendix} for more details about how to compute the bidding function. Table \ref{tb:counterfactual_winning_price_symmetric} and  \ref{tb:counterfactual_winning_price_asymmetric} display the expected revenue for each combination of tract size, auction format, participants, and consumption periods for each symmetric and asymmetric auction, respectively. In these tables, S refers to a sawmill, while L denotes a logger. For instance, (S, L) captures the competition where one sawmill and one logger compete. In Table \ref{tb:counterfactual_winning_price_symmetric}, I do not compute revenues in the sealed bid format, as the revenue equivalence theorem holds in symmetric auctions.  



\begin{table}[!htbp]
  \begin{center}
      \caption{Counterfactuals: expected revenue in symmetric auctions}
      \label{tb:counterfactual_winning_price_symmetric} 
       \subfloat[Small Tract Size]{\input{figuretable/counterfactual_winning_price_symmetric_small_tract}}\\
      \subfloat[Large Tract Size]{\input{figuretable/counterfactual_winning_price_symmetric_large_tract}}
  \end{center}\footnotesize
  \textit{Note}: Panels (a) and (b) display the average revenue for each counterfactual scenario involved with small and large tracts, respectively. In the ``Participants'' column, S (L) represents a sawmill (logger). The fourth to seventh column captures the contract length. All values are reported in 1,000 USD.
\end{table} 

\begin{table}[!htbp]
  \begin{center}
      \caption{Counterfactuals: expected revenue in asymmetric auctions}
      \label{tb:counterfactual_winning_price_asymmetric} 
       \subfloat[Small Tract Size]{\input{figuretable/counterfactual_winning_price_asymmetric_small_tract}}\\
      \subfloat[Large Tract Size]{\input{figuretable/counterfactual_winning_price_asymmetric_large_tract}}
  \end{center}\footnotesize
  \textit{Note}: Panels (a) and (b) display the average revenue for each counterfactual scenario involved with small and large tracts, respectively. In the ``Participants'' column, S (L) represents a sawmill (logger). The fourth to seventh column captures the contract length. All values are reported in 1,000 USD.
\end{table} 




Our counterfactual analyses in Table \ref{tb:counterfactual_winning_price_symmetric} indicate that extending the consumption periods—from, for example, 4 to 16 quarters—consistently increases expected revenues in symmetric settings. In Table 8, panel (a), with two identical Sawmills (S,S) operating under a small tract, revenue rises from approximately 152.8 at 4 quarters to about 290.4 at 16 quarters, a gain of roughly 90\%. Similarly, for two-logger case (L,L) in Table \ref{tb:counterfactual_winning_price_symmetric}, panel (a), revenue grows from about 73.7 to 84.1, an increase of about 14\%. Although the magnitude differs by bidder type, the central insight remains: providing buyers more temporal flexibility to align consumption timing with market conditions generally elevates their willingness-to-pay, thereby increasing revenues.

Although extending the consumption periods boosts revenues, intensifying competition among symmetric bidders can attenuate the relative growth rate. To see this, compare the (S,S) configuration (two identical Sawmill bidders) against the (S,S,S) configuration (three identical Sawmill bidders) in Table \ref{tb:counterfactual_winning_price_symmetric}, panel (a). With (S,S), extending the consumption periods from 4 to 16 quarters increases revenues by about 90\% (from approximately 152.8 to 290.4). In contrast, adding an additional Sawmill to create (S,S,S) still raises revenues substantially—from about 165.9 at 4 quarters to roughly 308.5 at 16 quarters—but the percentage increase (approximately 86\%) is slightly lower. In other words, when competition becomes more intense, much of the product’s value is already capitalized at shorter horizons due to aggressive bidding among identical, high-type participants. The incremental advantage of extended consumption windows, while still present, yields relatively smaller percentage gains because the heightened competitive pressure already elevates the baseline (4-quarter) revenue level.


When bidders are not symmetric—such as in combinations of sawmills (S) and loggers (L)—the general patterns observed in the symmetric scenarios do not directly apply. In these settings, the revenue equivalence theorem does not hold, and the choice between sealed-bid and oral auctions becomes more consequential. A key observation is that loggers typically exhibit a weaker incremental valuation from longer consumption periods relative to sawmills. This asymmetry in valuation growth under extended horizons affects how each auction format translates underlying valuations into final revenues. Table \ref{tb:counterfactual_winning_price_asymmetric} presents these asymmetric conditions.

\begin{figure}[!ht]
  \begin{center}
 % \subfloat[Cutting stage \textcolor{blue}{[TBA]}]{\includegraphics[keepaspectratio, scale=0.6]{figuretable/model_fit_bidder_valuation_highest_bid.png}}
   \subfloat[Two-bidder case]{\includegraphics[keepaspectratio, scale=0.5]{figuretable/counterfactual_bidding_function/counterfactual_auction_13quarters_type1_sawmill_type2_logger.png}}
   \subfloat[Three-bidder case]{\includegraphics[keepaspectratio, scale=0.5]{figuretable/counterfactual_bidding_function/counterfactual_auction_13quarters_type1_sawmill_type2_sawmill_type3_logger.png}}
  \caption{Bidding functions}
  \label{fg:counterfactual_bidding_function_asymmetric} 
  \end{center}
  \footnotesize
  Note: See Appendix \ref{sec:appendix} for more details about how to compute the bidding function.
\end{figure} 

Panel (a) in Table \ref{tb:counterfactual_winning_price_asymmetric} suggests that in a (S,L) scenario, shifting from 4 to 16 quarters under a sealed-bid format can produce relatively larger proportional increases in expected revenue than under an oral format: 13.6\% (from 78.0 to 88.7) increase under oral auction while 16.1\% (from 84.2 to 97.7) increase under sealed-bid auction. This occurs because the oral auction’s final price often aligns with the second-highest valuation, which in this case is likely the logger’s lower incremental valuation. As a result, the oral auction’s revenue growth is muted. By contrast, the sealed-bid environment, starting from a lower baseline due to bid shading, can reflect even modest valuation increases more prominently, leading to a higher percentage gain. We plot the bidding function in the sealed-bid auctions in Figure \ref{fg:counterfactual_bidding_function_asymmetric}, indicating that sawmills, as stronger bidders, shade bids more, and this behavior is mitigated when they face a more competitive environment. 


Now consider a (S,S,L) configuration in Table \ref{tb:counterfactual_winning_price_asymmetric}, panel (a), with a small tract. The extension from 4 to 16 quarters raises oral auction revenues from about 152.8 to 290.4 (+90\%), while sealed-bid revenues grow from roughly 154.3 to 238.0 (+54\%). In contrast with the (S,L) case, this configuration suggests that oral auction can strengthen the revenue-enhancing effect of a longer consumption period. In a (S,S,L) configuration, the second-highest bidder is more likely to be a sawmill, whose incremental valuation with a longer consumption period is stronger. Consequently, the oral format, which surfaces the second-highest valuation more effectively, exhibits more substantial revenue growth. Meanwhile, the sealed-bid format, involving shading bids, provides fewer opportunities for valuations to converge toward the second-highest bidder’s higher incremental valuation, resulting in comparatively smaller gains. Similar patterns show up in a large tract, and these findings highlight that when bidders differ in how they value extended consumption periods, the interplay between auction format and bidder composition critically influences the degree to which longer horizons translate into higher revenues.


An important additional factor is tract size. In both symmetric and asymmetric cases, larger tracts can magnify the revenue benefits of extended consumption periods. For instance, in Table \ref{tb:counterfactual_winning_price_symmetric}, panel (b), the (S,S) scenario shows a dramatic expansion, from about 103.3 at 4 quarters to roughly 455.0 at 16 quarters, a surge of more than 300\%. By contrast, the small tract scenario (Table \ref{tb:counterfactual_winning_price_asymmetric}, panel (a)) for (S,S) produced a 90\% increase—substantial, but markedly smaller. Similarly, in asymmetric settings (Table \ref{tb:counterfactual_winning_price_asymmetric}, panel (b)), large tracts amplify absolute gains because the greater underlying resource value makes timing options more potent. Both S and L bidders can benefit, though not equally, and the resulting changes in valuation further depend on whether the auction format encourages or mitigates strategic shading.

In summary, these counterfactual results reveal that the positive impact of lengthening the consumption periods on expected revenues is robust yet contingent upon multiple factors. The number of interested buyers, the composition of these buyers, the auction format, and the tract size all interact to shape how effectively extended horizons translate into final revenue. For managers and policymakers designing advance selling strategies, these insights underscore the importance of aligning contract structures not only with buyer type composition and market thickness but also with the scale of the underlying product and lumber price environment.




==> text_sections/06_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
This study investigates the role of the consumption period—an integral component of advance selling contexts—using empirical evidence from U.S. timber auctions. We begin by documenting that, under the finite contractual horizons, buyers frequently utilize their rights close to the consumption deadline. This finding suggests that limited contract length can act as a binding constraint, preventing buyers from optimally timing their resource extraction to market conditions. By extending the consumption periods, buyers gain additional temporal flexibility, which translates into increased asset valuations at the time of purchase.

Through counterfactual simulations, we quantify the extent to which lengthening the consumption periods enhances buyers' valuations, and how these valuation increases pass through into higher seller revenues via competitive bidding. Our analysis shows that the magnitude of these effects depends on buyer heterogeneity (e.g., loggers vs. sawmills), auction format (oral vs. sealed-bid), and the underlying uncertainty over future market demand. These findings hold practical implications: when sellers have limited knowledge of the distribution of future buyers' valuations under demand uncertainty, auctions can serve as a mechanism to reveal willingness-to-pay. The results suggest that, by carefully setting the consumption periods and choosing the appropriate auction design, sellers can improve their expected revenue even without perfect foresight into market conditions or buyer preferences.

At the same time, several caveats remain. We abstract from considerations of bidder risk aversion, implicitly treating players as risk-neutral. Incorporating risk preferences could alter both valuation and bidding behavior, potentially affecting the net benefit of extending consumption periods. Furthermore, our analysis focuses on how contract length affects buyers' valuations and, ultimately, seller revenues, but does not account for potential costs to the seller associated with extending the consumption periods due to the lack of data. In the context of timber sales, such costs might include heightened environmental impacts, increased risk of wildfires, or other long-term management challenges that arise when timbers remain unharvested for longer. Accounting for these trade-offs would provide a more complete picture of the net welfare implications and inform policy decisions in natural resource markets.

In sum, this paper contributes to the advance selling literature by highlighting the strategic importance of the consumption period’s length, demonstrating how it interacts with market uncertainty, auction formats, and bidder heterogeneity to shape outcomes. Our findings open avenues for future research to incorporate risk preferences and additional seller-side considerations, ultimately offering a richer framework for understanding and designing advance selling mechanisms in various market environments. For future research, it would be valuable to explore the optimal contract length that balances the marginal expected revenue and the marginal cost of extending the contract term, akin to the analyses found in the literature on optimal patent length.
